Non-Deterministic Functions as Non-Deterministic Processes (Extended Version)

We study encodings of the lambda-calculus into the pi-calculus in the unexplored case of calculi with non-determinism and failures. On the sequential side, we consider lambdafail, a new non-deterministic calculus in which intersection types control resources (terms); on the concurrent side, we consider spi, a pi-calculus in which non-determinism and failure rest upon a Curry-Howard correspondence between linear logic and session types. We present a typed encoding of lambdafail into spi and establish its correctness. Our encoding precisely explains the interplay of non-deterministic and fail-prone evaluation in lambdafail via typed processes in spi. In particular, it shows how failures in sequential evaluation (absence/excess of resources) can be neatly codified as interaction protocols.

==> figure.tex <==
 \tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp7964522619162369] 
\draw   (22,105.25) .. controls (22,85.78) and (37.78,70) .. (57.25,70) .. controls (76.72,70) and (92.5,85.78) .. (92.5,105.25) .. controls (92.5,124.72) and (76.72,140.5) .. (57.25,140.5) .. controls (37.78,140.5) and (22,124.72) .. (22,105.25) -- cycle ;
%Shape: Circle [id:dp2429873823346096] 
\draw   (186.5,105.5) .. controls (186.5,86.17) and (202.17,70.5) .. (221.5,70.5) .. controls (240.83,70.5) and (256.5,86.17) .. (256.5,105.5) .. controls (256.5,124.83) and (240.83,140.5) .. (221.5,140.5) .. controls (202.17,140.5) and (186.5,124.83) .. (186.5,105.5) -- cycle ;
%Shape: Circle [id:dp9380332011019401] 
\draw   (104,223) .. controls (104,200.36) and (122.36,182) .. (145,182) .. controls (167.64,182) and (186,200.36) .. (186,223) .. controls (186,245.64) and (167.64,264) .. (145,264) .. controls (122.36,264) and (104,245.64) .. (104,223) -- cycle ;
%Shape: Circle [id:dp34779892344880925] 
\draw   (132,212) .. controls (132,200.95) and (140.95,192) .. (152,192) .. controls (163.05,192) and (172,200.95) .. (172,212) .. controls (172,223.05) and (163.05,232) .. (152,232) .. controls (140.95,232) and (132,223.05) .. (132,212) -- cycle ;
%Straight Lines [id:da4684388085916382] 
\draw    (79,105) -- (199.5,106.48) ;
\draw [shift={(201.5,106.5)}, rotate = 180.7] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da836225068889987] 
\draw    (211.5,127) -- (156.64,206.35) ;
\draw [shift={(155.5,208)}, rotate = 304.65999999999997] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da16098165722112578] 
\draw    (74.5,126.5) -- (148.14,206.03) ;
\draw [shift={(149.5,207.5)}, rotate = 227.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (48.5,96.4) node [anchor=north west][inner sep=0.75pt]    {$\lamrfail$};
% Text Node
\draw (215,97.4) node [anchor=north west][inner sep=0.75pt]    {$\lamrsharfail$};
% Text Node
\draw (117,224.9) node [anchor=north west][inner sep=0.75pt]    {$\spi$};
% Text Node
\draw (121,17.9) node [anchor=north west][inner sep=0.75pt]    {$
                                                                    \begin{aligned}
                                                                        \text{Thm }  \ref{thm:preservencintolamrfail2}\\
                                                                        \text{Thm } \ref{l:app_completenessone}\\
                                                                        \text{Thm } \ref{l:soundnessone}\\
                                                                        \text{Thm } \ref{proof:app_successsensce}\\
                                                                    \end{aligned}$};
% Text Node
\draw (203,152.9) node [anchor=north west][inner sep=0.75pt]    {$
                                                                    \begin{aligned}
                                                                        \text{Thm }  \ref{t:preservationtwo}\\
                                                                        \text{Thm } \ref{l:app_completenesstwo}\\
                                                                        \text{Thm } \ref{l:app_soundnesstwo}\\
                                                                        \text{Thm } \ref{proof:successsenscetwo}\\
                                                                    \end{aligned}$};


\end{tikzpicture}
